ScaleLLM: A Resource-Frugal LLM Serving Framework by Optimizing End-to-End Efficiency

Large language models (LLMs) have surged in popularity and are extensively used in commercial applications, where the efficiency of model serving is crucial for the user experience. Most current research focuses on optimizing individual sub-procedures, e.g. local inference and communication, however, there is no comprehensive framework that provides a holistic system view for optimizing LLM serving in an end-to-end manner. In this work, we conduct a detailed analysis to identify major bottlenecks that impact end-to-end latency in LLM serving systems. Our analysis reveals that a comprehensive LLM serving endpoint must address a series of efficiency bottlenecks that extend beyond LLM inference. We then propose ScaleLLM, an optimized system for resource-efficient LLM serving. Our extensive experiments reveal that with 64 concurrent requests, ScaleLLM achieves a 4.3x speed up over vLLM and outperforms state-of-the-arts with 1.5x higher throughput.

==> tables/comparisons_with_state_of_the_arts.tex <==


\begin{table*}[t]
\centering
\caption{Comparison of Optimizations with State-of-the-art Serving Frameworks. \shanshan{To Raphael and Alay: could you fill this table}}
\label{tbl:comparison}
\begin{tabular}{c|l|c|c|c}
\toprule
 & \textbf{Optimization} &\textbf{HF Transformers} & \textbf{vLLM} & \textbf{ScaleLLM (Ours)} \\ 
\midrule
\multirow{4}{1.5cm}{\textbf{Serving Engine}} 
% \cmidrule{1-1}
&Continuous Batching &  & \greencmark & \greencmark  \\ \cmidrule{2-5}
&Quantization & \greencmark & \greencmark & \greencmark \\ \cmidrule{2-5}
&Expert Parallelism &  &  & \greencmark\\ \cmidrule{2-5}
&Operator Fusion &  & \greencmark & \greencmark\\ \hline
\multirow{3}{1.5cm}{\textbf{Gateway}}
&Reusable Connection Pool &  &  & \greencmark \\ \cmidrule{2-5}
&Multi-core CPU Utilization &  &  & \greencmark \\ \cmidrule{2-5}
&Dynamic Routing &  &  & \greencmark \\ 
&Dynamic Routing &  &  & \greencmark \\ 
\bottomrule
\end{tabular}
\end{table*}



% \begin{table*}[t]
%   \centering
%   \footnotesize
%   \caption{The resolution mechanism implementation differences of mainstream DNS software for recursives.}
%   \vspace{-4mm}
%   \begin{threeparttable}
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%     \toprule
%     \multirow{2}[3]{*}{\textbf{Software}} & \multirow{2}[3]{*}{\textbf{Version}} & \textbf{Answer} & \textbf{Referral} & \textbf{Cache update} & \textbf{Max} & \textbf{Max} & \textbf{Query} & \multirow{2}[3]{*}{\textbf{0x20}} & \multirow{2}[3]{*}{\textbf{DNSSEC}} & \multicolumn{5}{c}{\textbf{Vulnerable}} \\
%     \cmidrule{11-15}          &       & \textbf{data}\tnote{1} & \textbf{data}\tnote{1} & \textbf{policy} & \textbf{TTL} & \textbf{timeout} & \textbf{count} &       &       & aaa & bbb & ccc & ddd & eee \\
%     \midrule
%     BIND9~\cite{bind} & 9.18.1\tnote{2} & \cmark & \cmark & Child-centric & 7 days & 10s   & 13    & \xmark & \cmark & \greenxmark & \redcmark\color{black}\tnote{3} & \redcmark & \redcmark\color{black}\tnote{3} & \redcmark \\
%     \midrule
%     Knot Resolver~\cite{knot} & 5.5.0 & \cmark & \cmark & Child-centric & 6 days & 1.2s  & 3     & \cmark & \cmark & \redcmark\color{black}\tnote{4} & \redcmark & \redcmark & \redcmark & \redcmark \\
%     \midrule
%     Unbound~\cite{unbound} & 1.15.0 & \cmark & \cmark & Child-centric & 1 day & >10s\tnote{5} & 9     & \cmark & \cmark & \greenxmark & \redcmark & \redcmark & \redcmark & \redcmark \\
%     \midrule
%     PowerDNS Recursor~\cite{powerdns} & 4.6.2 & \cmark & \cmark & Child-centric & 1 day & 1.5s  & 1     & \cmark & \cmark & \greenxmark & \greenxmark & \greenxmark & \redcmark & \redcmark \\
%     \midrule
%     Microsoft DNS~\cite{msdns}\tnote{6} & 2022  & \cmark & \cmark & Parent-centric & 1 day & 3s    & 1     & \cmark & \cmark & \greenxmark & \greenxmark & \greenxmark & \redcmark & \redcmark\color{black}\tnote{7} \\
%     \midrule
%     Simple DNS Plus~\cite{simpledns} & 9.1   & \cmark & \cmark & Parent-centric & 7 days & 1.5s  & 3     & \cmark & \cmark & \greenxmark & \greenxmark & \greenxmark & \redcmark & \redcmark\color{black}\tnote{7} \\
%     \midrule
%     Technitium~\cite{technitium} & 8.0.2 & \xmark & \cmark & Parent-centric & 7 days & 10s   & 6     & \cmark & \cmark & \greenxmark & \greenxmark & \redcmark\color{black}\tnote{8,9} & \greenxmark & \redcmark\color{black}\tnote{9} \\
%     \midrule
%     MaraDNS~\cite{maradns} & 3.5.0021 & \xmark & \cmark & Parent-centric & 1 day & 6s    & 6     & \cmark & \xmark & \greenxmark & \greenxmark & \greenxmark & \greenxmark & \redcmark\color{black}\tnote{7} \\
%     \bottomrule
%     \end{tabular}%
%     \begin{tablenotes}
%         \footnotesize
%         \item[1] Whether caching delegation data of the authoritative section (\texttt{NS} records) and additional (glue records) section from answer or referral responses.
%         \item[2] BIND Version 9.16.27 is vulnerable as well and its maximum query number is 6. 
%         \item[3] Not vulnerable if the DNSSEC option is turned on.
%         \item[4] Vulnerable if the remaining TTL value is $\leq$ 5s or 1\% of original TTL.
%         \item[5] The maximum timeout of Unbound is about 46x RTT (round-trip-time).
%         \item[6] The maximum label number of Microsoft DNS is 39, while the others are limited by the maximum domain name length (255) and label length (63).
%         \item[7] Vulnerable if delegating to a new IP address.
%         \item[8] Vulnerable if delegating to a new \texttt{NS} name different from the query domain name.
%         \item[9] Still vulnerable if the \texttt{NS} Revalidation option is turned on, which is turned off by default.
%     \end{tablenotes}
%   \end{threeparttable}
%   \label{tab:software_summary}%
% \end{table*}%




% \begin{table*}[ht]
% \centering
% \captionsetup{justification=centering}
% \caption{Comparison of Optimizations with State-of-the-art Serving Frameworks}
% \label{table:comparison}
% \begin{tabular}{p{2.5cm}|p{5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}}
% \toprule
%  & \textbf{Source of Latency} & \textbf{HF Transformers} & \textbf{vLLM} & \textbf{TensorRT} & \textbf{Ours} \\ 
% \midrule
% \multirow{4}{2cm}{\textbf{Serving Engine}} 
% & Inference Computation &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Resource Management &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Batching and Parallelism &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Memory Management &  &  &  & \greencmark \\ 
% \midrule
% \multirow{4}{2cm}{\textbf{Gateway}} 
% & Request Routing &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Network Communication &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Security and Authentication &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Fault Tolerance &  &  &  & \greencmark \\ 
% \midrule
% \multirow{2}{2cm}{\textbf{Combined Factors}}
% & Concurrency Management &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Scalability Issues &  &  &  & \greencmark \\ 
% \bottomrule
% \end{tabular}
% \end{table*}

==> tables/throughput.tex <==
\begin{table*}[t]
\centering
\caption{TTFT and TBT}
\label{tbl:comparison}
\begin{tabular}{l|cc|cc|cc}
\toprule
\textbf{Concurrency} & \multicolumn{2}{c|}{\textbf{HF Transformers}} & \multicolumn{2}{c|}{\textbf{vLLM}} & \multicolumn{2}{c}{\textbf{ScaleLLM (Ours)}} \\ 
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}
& TTFT/ms & TBT/ms & TTFT/ms  & TBT/ms  & TTFT/ms  & TBT/ms  \\
\midrule
1 & 315.6 & 83.4 & 48.4 & 16.5 & 25.0 & 8.5 \\ 
2 & 637.2 & 218.3 & 51.9 & 16.7 & 25.3 & 8.7 \\ 
4 & 1157.8 & 506.4 & 55.1 & 21.1 & 25.5 & 10.4 \\ 
8 & - & - & 70.2 & 30.1 & 25.9 & 12.2 \\
16 & - & - & 93.1 & 38.3 & 26.7 & 13.4 \\ 
32 & - & - & 135.8 & 50.1 & 29.8 & 14.6 \\ 
64 & - & - & 285.4 & 70.8 & 99.4 & 16.5 \\ 
128 & - & - & 512.7 & 108.7 & 542.6 & 20.6 \\
256 & - & - & 634.0 & 175.8 & 2030.7 & 20.75 \\
\bottomrule
\end{tabular}
\end{table*}

% \begin{table*}[t]
%   \centering
%   \footnotesize
%   \caption{The resolution mechanism implementation differences of mainstream DNS software for recursives.}
%   \vspace{-4mm}
%   \begin{threeparttable}
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
%     \toprule
%     \multirow{2}[3]{*}{\textbf{Software}} & \multirow{2}[3]{*}{\textbf{Version}} & \textbf{Answer} & \textbf{Referral} & \textbf{Cache update} & \textbf{Max} & \textbf{Max} & \textbf{Query} & \multirow{2}[3]{*}{\textbf{0x20}} & \multirow{2}[3]{*}{\textbf{DNSSEC}} & \multicolumn{5}{c}{\textbf{Vulnerable}} \\
%     \cmidrule{11-15}          &       & \textbf{data}\tnote{1} & \textbf{data}\tnote{1} & \textbf{policy} & \textbf{TTL} & \textbf{timeout} & \textbf{count} &       &       & aaa & bbb & ccc & ddd & eee \\
%     \midrule
%     BIND9~\cite{bind} & 9.18.1\tnote{2} & \cmark & \cmark & Child-centric & 7 days & 10s   & 13    & \xmark & \cmark & \greenxmark & \redcmark\color{black}\tnote{3} & \redcmark & \redcmark\color{black}\tnote{3} & \redcmark \\
%     \midrule
%     Knot Resolver~\cite{knot} & 5.5.0 & \cmark & \cmark & Child-centric & 6 days & 1.2s  & 3     & \cmark & \cmark & \redcmark\color{black}\tnote{4} & \redcmark & \redcmark & \redcmark & \redcmark \\
%     \midrule
%     Unbound~\cite{unbound} & 1.15.0 & \cmark & \cmark & Child-centric & 1 day & >10s\tnote{5} & 9     & \cmark & \cmark & \greenxmark & \redcmark & \redcmark & \redcmark & \redcmark \\
%     \midrule
%     PowerDNS Recursor~\cite{powerdns} & 4.6.2 & \cmark & \cmark & Child-centric & 1 day & 1.5s  & 1     & \cmark & \cmark & \greenxmark & \greenxmark & \greenxmark & \redcmark & \redcmark \\
%     \midrule
%     Microsoft DNS~\cite{msdns}\tnote{6} & 2022  & \cmark & \cmark & Parent-centric & 1 day & 3s    & 1     & \cmark & \cmark & \greenxmark & \greenxmark & \greenxmark & \redcmark & \redcmark\color{black}\tnote{7} \\
%     \midrule
%     Simple DNS Plus~\cite{simpledns} & 9.1   & \cmark & \cmark & Parent-centric & 7 days & 1.5s  & 3     & \cmark & \cmark & \greenxmark & \greenxmark & \greenxmark & \redcmark & \redcmark\color{black}\tnote{7} \\
%     \midrule
%     Technitium~\cite{technitium} & 8.0.2 & \xmark & \cmark & Parent-centric & 7 days & 10s   & 6     & \cmark & \cmark & \greenxmark & \greenxmark & \redcmark\color{black}\tnote{8,9} & \greenxmark & \redcmark\color{black}\tnote{9} \\
%     \midrule
%     MaraDNS~\cite{maradns} & 3.5.0021 & \xmark & \cmark & Parent-centric & 1 day & 6s    & 6     & \cmark & \xmark & \greenxmark & \greenxmark & \greenxmark & \greenxmark & \redcmark\color{black}\tnote{7} \\
%     \bottomrule
%     \end{tabular}%
%     \begin{tablenotes}
%         \footnotesize
%         \item[1] Whether caching delegation data of the authoritative section (\texttt{NS} records) and additional (glue records) section from answer or referral responses.
%         \item[2] BIND Version 9.16.27 is vulnerable as well and its maximum query number is 6. 
%         \item[3] Not vulnerable if the DNSSEC option is turned on.
%         \item[4] Vulnerable if the remaining TTL value is $\leq$ 5s or 1\% of original TTL.
%         \item[5] The maximum timeout of Unbound is about 46x RTT (round-trip-time).
%         \item[6] The maximum label number of Microsoft DNS is 39, while the others are limited by the maximum domain name length (255) and label length (63).
%         \item[7] Vulnerable if delegating to a new IP address.
%         \item[8] Vulnerable if delegating to a new \texttt{NS} name different from the query domain name.
%         \item[9] Still vulnerable if the \texttt{NS} Revalidation option is turned on, which is turned off by default.
%     \end{tablenotes}
%   \end{threeparttable}
%   \label{tab:software_summary}%
% \end{table*}%




% \begin{table*}[ht]
% \centering
% \captionsetup{justification=centering}
% \caption{Comparison of Optimizations with State-of-the-art Serving Frameworks}
% \label{table:comparison}
% \begin{tabular}{p{2.5cm}|p{5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}}
% \toprule
%  & \textbf{Source of Latency} & \textbf{HF Transformers} & \textbf{vLLM} & \textbf{TensorRT} & \textbf{Ours} \\ 
% \midrule
% \multirow{4}{2cm}{\textbf{Serving Engine}} 
% & Inference Computation &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Resource Management &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Batching and Parallelism &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Memory Management &  &  &  & \greencmark \\ 
% \midrule
% \multirow{4}{2cm}{\textbf{Gateway}} 
% & Request Routing &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Network Communication &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Security and Authentication &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Fault Tolerance &  &  &  & \greencmark \\ 
% \midrule
% \multirow{2}{2cm}{\textbf{Combined Factors}}
% & Concurrency Management &  &  &  & \greencmark \\ \cmidrule{2-6}
% & Scalability Issues &  &  &  & \greencmark \\ 
% \bottomrule
% \end{tabular}
% \end{table*}
